Reachability and Matching in Single Crossing Minor Free Graphs

We show that for each single crossing graph $H$, a polynomially bounded weight function for all $H$-minor free graphs $G$ can be constructed in Logspace such that it gives nonzero weights to all the cycles in $G$. This class of graphs subsumes almost all classes of graphs for which such a weight function is known to be constructed in Logspace. As a consequence, we obtain that for the class of $H$-minor free graphs where $H$ is a single crossing graph, reachability can be solved in UL, and bipartite maximum matching can be solved in SPL, which are small subclasses of the parallel complexity class NC. In the restrictive case of bipartite graphs, our maximum matching result improves upon the recent result of Eppstein and Vazirani, where they show an NC bound for constructing perfect matching in general single crossing minor free graphs.

==> iso.tex <==
\section{Dynamic isolation from static non-zero circulation}\label{sec:iso}
In  previous sections, we have shown that we can compute a non-zero
circulation (for Matchings) in a bipartite single crossing minor free graph 
in $\L$. This allows us to compute if the graph has a perfect matching 
in $\SPL \subseteq \NC$.

In the dynamic setting, we allow the graph to evolve by insertion and 
deletion of a small number of edges at every time step under the promise 
that the graph stays $H$-minor free for a fixed single crossing graph $H$. 
We would like to maintain if the graph has a perfect matching in $\DynFO$.
One plausible approach would be to maintain the non-zero circulation as
described in Section~\ref{sec:wtfn}.
However, this seems non-trivial as we would need to maintain the decomposition
of the given graph into planar and constant tree-width parts in $\DynFO$. Even
if we could somehow do that, the weight of many edges may change due to 
even a single edge change. Thus many more than polylog many entries of the
adjacency and Tutte matrices may change. This would preclude the use of ``small
change'' techniques like the Sherman-Morrison-Woodbury formula.
This induces us to side-step the update of the non-zero
circulation by the method of Section~\ref{sec:wtfn}.

Instead we use a result from \cite{FGT} to convert the given static circulation
to  dynamic isolating weights. Notice that \cite{FGT} yields a black box recipe
to produce isolating weights of quasipolynomial magnitude in the following way.
Given a bipartite graph $G$, they first consider a non-zero circulation
of exponential magnitude viz. $w_0(e) : e \mapsto 2^e$. Next, they consider a 
list of $\ell = O(\log{n})$ primes $\vec{p} = \left<p_,\ldots,p_{\ell}\right>$ 
which yield a weight function $w_{\vec{p}}(e)$. This is defined
by considering the $\ell$ weight functions 
$w_0\bmod{p_i}$ for $i \in \{1,\ldots,\ell\}$
and concatenating them after introducing a \emph{shift} in the bit
positions i.e.:
%$$w_{\vec{p}}(e) = \sum_{i=1}^{\ell}{(w_0(e) \bmod{p_i})B^{\ell-i}}$$
$w_{\vec{p}}(e) = \left<w_0(e) \bmod{p_1},\ldots,w_0(e) \bmod{p_\ell}\right>$.
%The number $B \geq n\max_{i=1}^\ell{p_i}$ is large enough so 
This is so that there is no
overflow from the $i$-th field to the $(i-1)$-st for any 
$i \in \{2,\ldots,\ell\}$. 

Suppose we start with a graph with static weights ensuring non-zero 
circulation. In a step, some edges are 
inserted or deleted. %There is no problem with deletions since the
%non-vanishing circulation remains as such after deletions since 
The graph after deletion is a subgraph of the original graph; hence the
non-zero circulation remains non-zero after a deletion\footnote{If we merely had isolating
weights this would not necessarily preserve isolation.}, but we have to do more
in the case of insertions. We aim to give the newly inserted edges FGT-weights
 (from \cite{FGT})
in the higher order bits while giving weight $0$ to all the original edges in 
$G$ again in the higher order bits. Thus the weight of all perfect matchings
that survive the deletions in a step remains unchanged. Moreover, if none such
survive but new perfect matchings are introduced (due to insertion of edges)
the lightest of them is determined solely by the weights of the newly
introduced edges. In this case, our modification of the existential proof 
from \cite{FGT} ensures that the minimum weight perfect matching is unique.
%% so that for different matchings the ordering is determined by the weights
%% of the new edges only if any new edges are included in either matchings but 
%% preserves the orderings of the old matchings. Thus the previously isolated
%% perfect matching will persist as the lightest if it existed (after the 
%% deletions) but if there is no such perfect matching
%% then a newly introduced perfect matching is 
%% isolated if it exists.

Notice that the FGT-recipe applied to a graph with polylog ($N = \log^{O(1)}{n}$)
edges yields
quasipolylogarithmically ($N^{\log^{O(1)}{N}}$) 
large weights which are therefore still subpolynomial ($2^{(\log{\log{n}})^{O(1)}} = 2^{o(\log{n})} = n^{o(1)}$).
Thus the weights remain polynomial when shifted to accommodate for the old 
weights. Further the number of primes is polyloglog ($\log^{O(1)}{N} = (\log{\log{n}})^{O(1)}$) and so sublogarithmic ($= \log^{o(1)}{n}$)
thus the number of possible different weights is subpolynomial hence our 
algorithm can be derandomized.

Before getting into technical details, we point out that in \cite{DKMTVZ20} a
similar scheme is used for reachability and bears the same relation to
\cite{KT16} as this section does to \cite{FGT}. We have the following lemma
, which we prove in Appendix~\ref{subsec:isoApp}:
\begin{lemma} \label{lem:combFGT}
Let $G$ be a bipartite graph with a non-zero circulation
$w$. Suppose $N = \log^{O(1)}{n}$ edges are inserted into $G$ to yield $G^{new}$
then we can compute polynomially many weight functions in $\FOar$ that
have $O(\log{n})$ bit weights, and at least one of them,
$w^{new}$ is isolating. Further the weights of the original edges remain
unchanged under $w^{new}$.
\end{lemma}



==> langDefs.tex <==
\subsection{Language Definitions}\label{subsec:langDefs}
\begin{definition}
\begin{itemize}
\item $\PM$ is a set of independent edges covering all the vertices of a graph. 
\item $\BPM$ is a $\PM$ in a bipartite graph.
\item $\PMD$ Given an undirected graph $G(V,E)$ determine if there exists a 
perfect matching in $G$.
\item $\PMS$ Construct a perfect matching for a given graph $G$ if one exists.
\item $\BMWPMS$ In an edge  weighted bipartite graph construct a $\PM$ of least weight.
\item $\MCM$ is a set of largest size consisting of independent edges.
\item $\BMCM$ is an $\MCM$ in a bipartite graph.
\item $\MWMCM$ is an $\MCM$ of least weight in an edge weighted graph.
\item $\BMWMCM$ is an $\MWMCM$ in a weighted bipartite graph.
\item $\MCMSz$ determine the size of an $\MCM$.
\item $\BMCMSz$ the $\MCMSz$ problem in bipartite graphs.
\item $\BMWMCMS$ Construct a $\BMWMCM$. 
\item $\Reach$ Given a directed graph $G(V,E)$ and $s,t \in V$ does there exist a directed path from $s$ to $t$ in $G$.
\item $\Dist$ Given a directed graph $G(V,E)$, polynomially bounded edge weights and $s,t \in V$ find the weight of a least weight path from $s$ to $t$.
\item $\Rank$ Given an $m \times n$  matrix $A$ with integer entries find 
the rank of $A$ over $\mathbb{Q}$.
\end{itemize}
\end{definition}


==> resultsTable.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\cline{1-6}
\multicolumn{2}{|c|}{} & \multicolumn{4}{c|}{Best Known Upperbound} \\
\cline{1-6}
\multicolumn{1}{|c|}{Graph} &
\multicolumn{1}{|c|}{Problem} & \multicolumn{1}{c}{Static}& \multicolumn{3}{|c|}{Dynamic (\#changes)}\\
\cline{4-6}
& & & $O(1)$ & $O(\frac{\log{n}}{\log{\log{n}}})$ & $\log^{O(1)}{n}$\\
\cline{1-6}
\multirow{4}{*}{Planar}
& ${\Reach}$		& $\UL\cap\coUL$\cite{TV12}   & $\DynFO$\cite{DKMSZ18} & $\DynFO$\cite{DMVZ18} & $\DynFOp$\cite{DKMTVZ20} \\
& $\Dist$ 	& $\UL\cap\coUL$\cite{TW10}	   & $\DynFOp$\cite{Mukherjee} & \framebox{$\DynFOp$} & \framebox{$\DynFOp$} \\
& $\BMCMSz$	& $\SPL$\cite{DKKM18}	   & \framebox{$\DynFO$} & \framebox{$\DynFO$} & \framebox{$\DynFOp$} \\
& $\BMCMS$	& $\SPL$\cite{DKKM18}	   & \framebox{$\DynFOp$} & \framebox{$\DynFOp$} & \framebox{$\DynFOp$} \\
\cline{1-6}
\multirow{4}{*}{SCMFree}
& $\Reach$	& \framebox{$\UL\cap\coUL$}   & $\DynFO$\cite{DKMSZ18} & $\DynFO$\cite{DMVZ18} & \framebox{$\DynFOp$} \\
&  $\Dist$ 	& \framebox{$\UL\cap\coUL$}	   & \framebox{$\DynFOp$} & \framebox{$\DynFOp$} & \framebox{$\DynFOp$} \\
& $\BMCMSz$	& \framebox{$\SPL$}	   & \framebox{$\DynFO$} & \framebox{$\DynFO$} & \framebox{$\DynFOp$} \\
& $\BMCMS$	& \framebox{$\SPL$}	   &  \framebox{$\DynFOp$} & \framebox{$\DynFOp$} & \framebox{$\DynFOp$} \\
\cline{1-6}
\end{tabular}
\caption{Previously known and \framebox{new} results in the static and the dynamic setting.}
\end{table}
%\begin{tabular}{|c|c||c|c|c|c|}
%\cline{1-6}
%\multicolumn{2}{|c||}{} & \multicolumn{4}{c|}{Best Upperbound} \\
%\cline{1-6}
%\multicolumn{1}{|c|}{Graph} &
%\multicolumn{1}{|c||}{Problem} & \multicolumn{1}{c}{Static}& \multicolumn{3}{|c|}{Dynamic (\#changes)}\\
%\cline{4-6}
%& & & $1$ & $O(\frac{\log{n}}{\log{\log{n}}})$ & $\log^{O(1)}{n}$\\
%\cline{1-6}
%\multirow{3}{*}{Planar}
%& Reach		& $\UL\cap\coUL$   & $\DynFO$ & $\DynFOar$ & $\DynFOpar$ \\
%& Bip PM Dec 	& $\SPL$	   & $\DynFO$? & $\DynFOar$? & $\DynFOpar$ \\
%& Bip PM Srch	& $\SPL$	   & $\DynFOp$? & $\DynFOpar$? & $\DynFOpar$ \\
%\cline{1-6}
%\multirow{3}{*}{SCM-Free}
%& Reach		& $\UL\cap\coUL$   & $\DynFO$ & $\DynFOar$ & $\DynFOpar$ \\
%& Bip PM Dec 	& $\SPL$	   & $\DynFO$? & $\DynFOar$? & $\DynFOpar$ \\
%& Bip PM Srch	& $\SPL$	   & $\DynFOp$? & $\DynFOpar$? & $\DynFOpar$ \\
%\cline{1-6}
%\end{tabular}
